U-Statistics for Importance-Weighted Variational Inference

We propose the use of U-statistics to reduce variance for gradient estimation in importance-weighted variational inference. The key observation is that, given a base gradient estimator that requires $m > 1$ samples and a total of $n > m$ samples to be used for estimation, lower variance is achieved by averaging the base estimator on overlapping batches of size $m$ than disjoint batches, as currently done. We use classical U-statistic theory to analyze the variance reduction, and propose novel approximations with theoretical guarantees to ensure computational efficiency. We find empirically that U-statistic variance reduction can lead to modest to significant improvements in inference performance on a range of models, with little computational cost.

==> autogenerated/average-diff-reduced-limits.tex <==
% this file was auto-generated
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                   measure \\
approxDist & model\_name & n &       &       &       &                           \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  1.29 &  4.23 &  4.72 &  complete-U - standard IW \\
                 & logistic-australian & 16 &  0.05 &  1.02 &  1.25 &  complete-U - standard IW \\
                 & logistic-ionosphere & 16 & -0.10 & -0.16 &  0.07 &  complete-U - standard IW \\
                 & logistic-madelon & 16 & 14.15 & 24.02 & 40.72 &  complete-U - standard IW \\
                 & logistic-mushrooms & 16 &  1.74 &  3.32 &  9.03 &  complete-U - standard IW \\
                 & logistic-sonar & 16 & -0.03 & -0.15 &  0.27 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                measure \\
approxDist & model\_name & n &       &       &       &                        \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  1.60 &  4.11 &  4.51 &  approx. - standard IW \\
                 & logistic-australian & 16 &  0.00 &  0.90 &  1.25 &  approx. - standard IW \\
                 & logistic-ionosphere & 16 & -0.17 & -0.29 & -0.13 &  approx. - standard IW \\
                 & logistic-madelon & 16 & 13.11 & 24.17 & 37.43 &  approx. - standard IW \\
                 & logistic-mushrooms & 16 &  1.56 &  3.29 &  8.54 &  approx. - standard IW \\
                 & logistic-sonar & 16 & -0.04 & -0.21 &  0.11 &  approx. - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                    measure \\
approxDist & model\_name & n &       &       &       &                            \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  1.49 &  4.08 &  4.45 &  approx. 2nd - standard IW \\
                 & logistic-australian & 16 &  0.05 &  0.96 &  1.28 &  approx. 2nd - standard IW \\
                 & logistic-ionosphere & 16 & -0.12 & -0.21 &  0.00 &  approx. 2nd - standard IW \\
                 & logistic-madelon & 16 & 13.53 & 22.75 & 40.73 &  approx. 2nd - standard IW \\
                 & logistic-mushrooms & 16 &  1.74 &  3.30 &  9.16 &  approx. 2nd - standard IW \\
                 & logistic-sonar & 16 & -0.02 & -0.18 &  0.15 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                       measure \\
approxDist & model\_name & n &       &       &       &                               \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  1.31 &  3.86 &  4.51 &  random subsets - standard IW \\
                 & logistic-australian & 16 & -0.00 &  0.96 &  1.24 &  random subsets - standard IW \\
                 & logistic-ionosphere & 16 & -0.06 & -0.12 &  0.06 &  random subsets - standard IW \\
                 & logistic-madelon & 16 & 14.41 & 23.97 & 35.69 &  random subsets - standard IW \\
                 & logistic-mushrooms & 16 &  1.19 &  3.66 &  7.05 &  random subsets - standard IW \\
                 & logistic-sonar & 16 & -0.02 & -0.17 &  0.17 &  random subsets - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                 measure \\
approxDist & model\_name & n &       &       &       &                         \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  1.54 &  4.01 &  4.48 &  permuted - standard IW \\
                 & logistic-australian & 16 &  0.02 &  1.00 &  1.38 &  permuted - standard IW \\
                 & logistic-ionosphere & 16 & -0.10 & -0.10 &  0.06 &  permuted - standard IW \\
                 & logistic-madelon & 16 & 14.94 & 21.27 & 37.30 &  permuted - standard IW \\
                 & logistic-mushrooms & 16 &  1.88 &  2.76 &  8.69 &  permuted - standard IW \\
                 & logistic-sonar & 16 &  0.03 & -0.15 &  0.19 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                 measure \\
approxDist & model\_name & n &       &       &       &                         \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  1.53 & 12.82 & 12.95 &  complete-U-DReG - DReG \\
                 & logistic-australian & 16 & -0.07 &  0.03 &  1.34 &  complete-U-DReG - DReG \\
                 & logistic-ionosphere & 16 & -0.11 & -0.12 &  0.23 &  complete-U-DReG - DReG \\
                 & logistic-madelon & 16 &  6.78 &  9.63 & 15.30 &  complete-U-DReG - DReG \\
                 & logistic-mushrooms & 16 &  2.45 &  4.41 &  7.97 &  complete-U-DReG - DReG \\
                 & logistic-sonar & 16 & -0.05 & -0.24 &  0.06 &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &               measure \\
approxDist & model\_name & n &       &       &       &                       \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  1.40 & 12.67 & 12.86 &  permuted-DReG - DReG \\
                 & logistic-australian & 16 & -0.07 &  0.06 &  1.43 &  permuted-DReG - DReG \\
                 & logistic-ionosphere & 16 & -0.12 & -0.08 &  0.31 &  permuted-DReG - DReG \\
                 & logistic-madelon & 16 &  7.42 &  9.14 & 14.49 &  permuted-DReG - DReG \\
                 & logistic-mushrooms & 16 &  1.94 &  4.69 &  8.50 &  permuted-DReG - DReG \\
                 & logistic-sonar & 16 &  0.03 & -0.28 &  0.21 &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                   measure \\
approxDist & model\_name & n &         &         &         &                           \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   47.55 &  105.74 &  122.37 &  complete-U - standard IW \\
                & logistic-australian & 16 &    1.34 &    2.72 &    3.51 &  complete-U - standard IW \\
                & logistic-ionosphere & 16 &    4.26 &   13.73 &   17.55 &  complete-U - standard IW \\
                & logistic-madelon & 16 & 2364.94 & 4527.06 & 7818.47 &  complete-U - standard IW \\
                & logistic-mushrooms & 16 &   67.38 &  153.48 &  214.68 &  complete-U - standard IW \\
                & logistic-sonar & 16 &   32.76 &   63.23 &   54.26 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                measure \\
approxDist & model\_name & n &         &         &         &                        \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   47.42 &  105.09 &  121.90 &  approx. - standard IW \\
                & logistic-australian & 16 &    1.00 &    2.23 &    2.91 &  approx. - standard IW \\
                & logistic-ionosphere & 16 &    3.98 &   13.32 &   17.01 &  approx. - standard IW \\
                & logistic-madelon & 16 & 2372.55 & 4526.01 & 7837.00 &  approx. - standard IW \\
                & logistic-mushrooms & 16 &   67.26 &  153.28 &  213.82 &  approx. - standard IW \\
                & logistic-sonar & 16 &   32.63 &   62.89 &   53.37 &  approx. - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                    measure \\
approxDist & model\_name & n &         &         &         &                            \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   47.53 &  105.30 &  122.34 &  approx. 2nd - standard IW \\
                & logistic-australian & 16 &    1.07 &    2.37 &    3.22 &  approx. 2nd - standard IW \\
                & logistic-ionosphere & 16 &    4.11 &   13.55 &   17.55 &  approx. 2nd - standard IW \\
                & logistic-madelon & 16 & 2371.55 & 4524.21 & 7828.81 &  approx. 2nd - standard IW \\
                & logistic-mushrooms & 16 &   67.28 &  153.58 &  214.31 &  approx. 2nd - standard IW \\
                & logistic-sonar & 16 &   32.94 &   63.34 &   54.14 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                       measure \\
approxDist & model\_name & n &         &         &         &                               \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   42.94 &   98.72 &  108.44 &  random subsets - standard IW \\
                & logistic-australian & 16 &    1.27 &    2.55 &    3.29 &  random subsets - standard IW \\
                & logistic-ionosphere & 16 &    3.67 &   12.93 &   15.69 &  random subsets - standard IW \\
                & logistic-madelon & 16 & 2104.95 & 4298.23 & 7568.27 &  random subsets - standard IW \\
                & logistic-mushrooms & 16 &   61.43 &  143.63 &  199.52 &  random subsets - standard IW \\
                & logistic-sonar & 16 &   27.86 &   59.85 &   48.81 &  random subsets - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                 measure \\
approxDist & model\_name & n &         &         &         &                         \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   45.36 &  100.56 &  112.42 &  permuted - standard IW \\
                & logistic-australian & 16 &    1.31 &    2.61 &    3.36 &  permuted - standard IW \\
                & logistic-ionosphere & 16 &    3.89 &   13.17 &   16.58 &  permuted - standard IW \\
                & logistic-madelon & 16 & 2275.40 & 4400.68 & 7691.99 &  permuted - standard IW \\
                & logistic-mushrooms & 16 &   64.46 &  145.85 &  202.56 &  permuted - standard IW \\
                & logistic-sonar & 16 &   30.15 &   61.09 &   50.62 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &     2 &      4 &      8 &                 measure \\
approxDist & model\_name & n &       &        &        &                         \\
\midrule
FullCovGaussian & logistic-a1a & 16 & 25.58 & 218.20 &  95.21 &  complete-U-DReG - DReG \\
                & logistic-australian & 16 &  1.46 &   1.91 &   3.96 &  complete-U-DReG - DReG \\
                & logistic-ionosphere & 16 &  4.56 &  17.08 &  20.36 &  complete-U-DReG - DReG \\
                & logistic-madelon & 16 &   NaN &    NaN &    NaN &  complete-U-DReG - DReG \\
                & logistic-mushrooms & 16 & 94.58 & 191.28 & 174.05 &  complete-U-DReG - DReG \\
                & logistic-sonar & 16 & 31.66 &  70.86 &  92.48 &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &     2 &      4 &      8 &               measure \\
approxDist & model\_name & n &       &        &        &                       \\
\midrule
FullCovGaussian & logistic-a1a & 16 & 27.30 & 111.74 & 119.51 &  permuted-DReG - DReG \\
                & logistic-australian & 16 &  1.45 &   1.87 &   3.94 &  permuted-DReG - DReG \\
                & logistic-ionosphere & 16 &  4.34 &  15.74 &  17.91 &  permuted-DReG - DReG \\
                & logistic-madelon & 16 &   NaN &    NaN &    NaN &  permuted-DReG - DReG \\
                & logistic-mushrooms & 16 & 93.45 & 186.01 & 179.02 &  permuted-DReG - DReG \\
                & logistic-sonar & 16 & 27.99 &  69.54 &  90.86 &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                   measure \\
approxDist & model\_name & n &       &        &       &                           \\
\midrule
DiagonalGaussian & congress & 16 &  2.90 &   4.89 &  7.71 &  complete-U - standard IW \\
                 & election88 & 16 &  0.14 &   2.79 &  7.15 &  complete-U - standard IW \\
                 & election88Exp & 16 &  4.73 & 117.76 & 55.28 &  complete-U - standard IW \\
                 & electric & 16 &  0.22 &   1.62 &  4.63 &  complete-U - standard IW \\
                 & electric-one-pred & 16 &  0.80 &  -0.72 & -4.33 &  complete-U - standard IW \\
                 & hepatitis & 16 &  2.10 & 156.63 &  1.89 &  complete-U - standard IW \\
                 & hiv-chr & 16 &  0.24 &   2.16 & 21.64 &  complete-U - standard IW \\
                 & irt & 16 &  0.22 &   0.84 &  1.20 &  complete-U - standard IW \\
                 & irt-multilevel & 16 & 29.77 &  54.47 & 52.93 &  complete-U - standard IW \\
                 & mesquite & 16 &  0.22 &   0.63 &  2.04 &  complete-U - standard IW \\
                 & radon & 16 &  7.50 &   9.02 & 63.74 &  complete-U - standard IW \\
                 & wells & 16 & -0.02 &   0.02 & -0.11 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                measure \\
approxDist & model\_name & n &       &        &       &                        \\
\midrule
DiagonalGaussian & congress & 16 &  2.76 &   4.73 &  7.39 &  approx. - standard IW \\
                 & election88 & 16 &  0.14 &   2.78 &  7.12 &  approx. - standard IW \\
                 & election88Exp & 16 &  4.73 & 117.73 & 55.07 &  approx. - standard IW \\
                 & electric & 16 &  0.09 &   1.44 &  4.24 &  approx. - standard IW \\
                 & electric-one-pred & 16 &  0.70 &  -0.82 & -4.49 &  approx. - standard IW \\
                 & hepatitis & 16 &  2.00 & 156.45 &  1.78 &  approx. - standard IW \\
                 & hiv-chr & 16 &  0.38 &   1.95 & 20.87 &  approx. - standard IW \\
                 & irt & 16 &  0.11 &   0.63 &  0.80 &  approx. - standard IW \\
                 & irt-multilevel & 16 & 31.28 &  45.44 & 59.92 &  approx. - standard IW \\
                 & mesquite & 16 & -0.08 &   0.11 &  1.43 &  approx. - standard IW \\
                 & radon & 16 &  7.45 &   8.70 & 63.51 &  approx. - standard IW \\
                 & wells & 16 & -0.26 &  -0.43 & -0.57 &  approx. - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                    measure \\
approxDist & model\_name & n &       &        &       &                            \\
\midrule
DiagonalGaussian & congress & 16 &  2.89 &   4.76 &  7.63 &  approx. 2nd - standard IW \\
                 & election88 & 16 &  0.12 &   2.84 &  7.06 &  approx. 2nd - standard IW \\
                 & election88Exp & 16 &  4.73 & 117.78 & 55.27 &  approx. 2nd - standard IW \\
                 & electric & 16 &  0.16 &   1.54 &  4.52 &  approx. 2nd - standard IW \\
                 & electric-one-pred & 16 &  0.74 &  -0.76 & -4.38 &  approx. 2nd - standard IW \\
                 & hepatitis & 16 &  2.06 & 156.53 &  1.86 &  approx. 2nd - standard IW \\
                 & hiv-chr & 16 &  0.34 &   2.12 & 21.74 &  approx. 2nd - standard IW \\
                 & irt & 16 &  0.15 &   0.72 &  0.93 &  approx. 2nd - standard IW \\
                 & irt-multilevel & 16 & 29.74 &  48.20 & 53.64 &  approx. 2nd - standard IW \\
                 & mesquite & 16 & -0.06 &   0.28 &  1.74 &  approx. 2nd - standard IW \\
                 & radon & 16 &  7.85 &   8.91 & 65.49 &  approx. 2nd - standard IW \\
                 & wells & 16 & -0.20 &  -0.30 & -0.35 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                       measure \\
approxDist & model\_name & n &       &        &       &                               \\
\midrule
DiagonalGaussian & congress & 16 &  2.45 &   4.17 &  7.10 &  random subsets - standard IW \\
                 & election88 & 16 &  0.37 &   2.46 &  6.62 &  random subsets - standard IW \\
                 & election88Exp & 16 &  5.30 & 104.62 & 43.10 &  random subsets - standard IW \\
                 & electric & 16 &  0.27 &   1.51 &  4.17 &  random subsets - standard IW \\
                 & electric-one-pred & 16 & -0.03 &  -0.29 & -3.26 &  random subsets - standard IW \\
                 & hepatitis & 16 & -0.31 &   1.69 &  1.60 &  random subsets - standard IW \\
                 & hiv-chr & 16 &  0.04 &   1.73 & 17.44 &  random subsets - standard IW \\
                 & irt & 16 &  0.25 &   0.86 &  0.96 &  random subsets - standard IW \\
                 & irt-multilevel & 16 & 35.73 &  27.61 & 46.49 &  random subsets - standard IW \\
                 & mesquite & 16 &  0.16 &   0.53 &  1.96 &  random subsets - standard IW \\
                 & radon & 16 &  7.81 &  18.19 & 28.92 &  random subsets - standard IW \\
                 & wells & 16 & -0.01 &   0.03 & -0.10 &  random subsets - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &     4 &     8 &                 measure \\
approxDist & model\_name & n &       &       &       &                         \\
\midrule
DiagonalGaussian & congress & 16 &  2.50 &  4.61 &  7.33 &  permuted - standard IW \\
                 & election88 & 16 &  0.12 &  2.66 &  6.94 &  permuted - standard IW \\
                 & election88Exp & 16 &  0.82 & 98.52 & 32.76 &  permuted - standard IW \\
                 & electric & 16 &  0.26 &  1.53 &  4.32 &  permuted - standard IW \\
                 & electric-one-pred & 16 &  0.66 & -0.77 & -3.91 &  permuted - standard IW \\
                 & hepatitis & 16 &  0.90 & -0.06 &  0.65 &  permuted - standard IW \\
                 & hiv-chr & 16 &  0.16 &  2.03 & 15.84 &  permuted - standard IW \\
                 & irt & 16 &  0.19 &  0.80 &  1.00 &  permuted - standard IW \\
                 & irt-multilevel & 16 & 35.69 & 43.79 & 62.32 &  permuted - standard IW \\
                 & mesquite & 16 &  0.20 &  0.58 &  2.00 &  permuted - standard IW \\
                 & radon & 16 &  7.88 &  5.79 & 14.83 &  permuted - standard IW \\
                 & wells & 16 & -0.02 &  0.01 & -0.11 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &      8 &                 measure \\
approxDist & model\_name & n &       &        &        &                         \\
\midrule
DiagonalGaussian & congress & 16 &  2.74 &   4.91 &   7.46 &  complete-U-DReG - DReG \\
                 & election88 & 16 &  0.15 &   2.61 &   7.20 &  complete-U-DReG - DReG \\
                 & election88Exp & 16 & 28.61 & 116.25 &  54.85 &  complete-U-DReG - DReG \\
                 & electric & 16 &  0.19 &   1.65 &   4.84 &  complete-U-DReG - DReG \\
                 & electric-one-pred & 16 &  0.81 &  -0.74 &  -4.32 &  complete-U-DReG - DReG \\
                 & hepatitis & 16 &  0.63 &   1.84 &   1.94 &  complete-U-DReG - DReG \\
                 & hiv-chr & 16 &  0.18 &   1.19 &  20.21 &  complete-U-DReG - DReG \\
                 & irt & 16 &  0.13 &   0.67 &   2.31 &  complete-U-DReG - DReG \\
                 & irt-multilevel & 16 & 51.16 &  65.97 &  52.09 &  complete-U-DReG - DReG \\
                 & mesquite & 16 &  0.07 &   0.51 &   1.96 &  complete-U-DReG - DReG \\
                 & radon & 16 &  8.15 &   9.76 & 117.37 &  complete-U-DReG - DReG \\
                 & wells & 16 & -0.02 &  -0.03 &  -0.15 &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &               measure \\
approxDist & model\_name & n &       &        &       &                       \\
\midrule
DiagonalGaussian & congress & 16 &  2.37 &   4.68 &  7.02 &  permuted-DReG - DReG \\
                 & election88 & 16 &  0.10 &   2.67 &  6.83 &  permuted-DReG - DReG \\
                 & election88Exp & 16 & -1.89 & 100.09 & 32.53 &  permuted-DReG - DReG \\
                 & electric & 16 &  0.24 &   1.56 &  4.63 &  permuted-DReG - DReG \\
                 & electric-one-pred & 16 &  0.69 &  -0.77 & -3.93 &  permuted-DReG - DReG \\
                 & hepatitis & 16 & -0.30 &   0.92 &  0.69 &  permuted-DReG - DReG \\
                 & hiv-chr & 16 & -0.08 &   1.45 & 12.91 &  permuted-DReG - DReG \\
                 & irt & 16 &  0.11 &   0.61 &  1.40 &  permuted-DReG - DReG \\
                 & irt-multilevel & 16 & 34.66 &  50.26 & 55.22 &  permuted-DReG - DReG \\
                 & mesquite & 16 & -0.29 &   0.39 &  1.99 &  permuted-DReG - DReG \\
                 & radon & 16 &  8.16 &   7.56 & 60.92 &  permuted-DReG - DReG \\
                 & wells & 16 & -0.02 &  -0.04 & -0.14 &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                   measure \\
approxDist & model\_name & n &       &         &        &                           \\
\midrule
FullCovGaussian & congress & 16 & 12.81 &   12.61 &  20.79 &  complete-U - standard IW \\
                & electric & 16 &   NaN &  -77.49 &  86.49 &  complete-U - standard IW \\
                & electric-one-pred & 16 & -3.18 &   -4.75 &  -4.35 &  complete-U - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  complete-U - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 320.80 &  complete-U - standard IW \\
                & mesquite & 16 &  2.68 &    1.32 &   1.48 &  complete-U - standard IW \\
                & radon & 16 &   NaN & 1317.59 & 304.34 &  complete-U - standard IW \\
                & wells & 16 &  0.01 &    0.06 &  -0.04 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                measure \\
approxDist & model\_name & n &       &         &        &                        \\
\midrule
FullCovGaussian & congress & 16 & 12.69 &   12.31 &  20.18 &  approx. - standard IW \\
                & electric & 16 &   NaN &  -85.03 &  90.40 &  approx. - standard IW \\
                & electric-one-pred & 16 & -3.20 &   -4.82 &  -4.46 &  approx. - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  approx. - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 322.27 &  approx. - standard IW \\
                & mesquite & 16 &  2.47 &    0.83 &   1.03 &  approx. - standard IW \\
                & radon & 16 &   NaN & 1313.61 & 306.69 &  approx. - standard IW \\
                & wells & 16 & -0.36 &   -0.44 &  -0.50 &  approx. - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                    measure \\
approxDist & model\_name & n &       &         &        &                            \\
\midrule
FullCovGaussian & congress & 16 & 12.33 &   12.57 &  20.46 &  approx. 2nd - standard IW \\
                & electric & 16 &   NaN &  -77.53 &  89.06 &  approx. 2nd - standard IW \\
                & electric-one-pred & 16 & -3.18 &   -4.77 &  -4.37 &  approx. 2nd - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  approx. 2nd - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 325.79 &  approx. 2nd - standard IW \\
                & mesquite & 16 &  2.43 &    0.95 &   1.19 &  approx. 2nd - standard IW \\
                & radon & 16 &   NaN & 1316.75 & 303.83 &  approx. 2nd - standard IW \\
                & wells & 16 & -0.29 &   -0.31 &  -0.29 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                       measure \\
approxDist & model\_name & n &       &         &        &                               \\
\midrule
FullCovGaussian & congress & 16 & 10.75 &   11.70 &  19.21 &  random subsets - standard IW \\
                & electric & 16 &   NaN & -181.35 &  86.60 &  random subsets - standard IW \\
                & electric-one-pred & 16 & -3.19 &   -5.35 &  -3.35 &  random subsets - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  random subsets - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 238.55 &  random subsets - standard IW \\
                & mesquite & 16 &  2.67 &    1.17 &   1.40 &  random subsets - standard IW \\
                & radon & 16 &   NaN & 1069.59 & 273.45 &  random subsets - standard IW \\
                & wells & 16 &  0.02 &    0.06 &  -0.04 &  random subsets - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                 measure \\
approxDist & model\_name & n &       &         &        &                         \\
\midrule
FullCovGaussian & congress & 16 & 11.62 &   12.02 &  19.80 &  permuted - standard IW \\
                & electric & 16 &   NaN &  -38.02 &  80.46 &  permuted - standard IW \\
                & electric-one-pred & 16 & -1.81 &   -4.73 &  -3.45 &  permuted - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  permuted - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 283.19 &  permuted - standard IW \\
                & mesquite & 16 &  2.57 &    1.20 &   1.41 &  permuted - standard IW \\
                & radon & 16 &   NaN & 1150.39 & 268.98 &  permuted - standard IW \\
                & wells & 16 &  0.02 &    0.07 &  -0.03 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                 measure \\
approxDist & model\_name & n &       &         &        &                         \\
\midrule
FullCovGaussian & congress & 16 & 14.98 &   13.56 &  21.80 &  complete-U-DReG - DReG \\
                & electric & 16 &   NaN &  -75.08 &  47.70 &  complete-U-DReG - DReG \\
                & electric-one-pred & 16 & -3.15 &   -4.75 &  -4.35 &  complete-U-DReG - DReG \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  complete-U-DReG - DReG \\
                & hiv-chr & 16 &   NaN &     NaN &    NaN &  complete-U-DReG - DReG \\
                & mesquite & 16 &  2.72 &    0.75 &   0.85 &  complete-U-DReG - DReG \\
                & radon & 16 &   NaN & 1349.19 & 320.94 &  complete-U-DReG - DReG \\
                & wells & 16 &  0.04 &    0.03 &  -0.02 &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &               measure \\
approxDist & model\_name & n &       &         &        &                       \\
\midrule
FullCovGaussian & congress & 16 & 13.55 &   13.11 &  20.96 &  permuted-DReG - DReG \\
                & electric & 16 &   NaN &  -43.16 &  34.91 &  permuted-DReG - DReG \\
                & electric-one-pred & 16 & -1.79 &   -4.72 &  -3.46 &  permuted-DReG - DReG \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  permuted-DReG - DReG \\
                & hiv-chr & 16 &   NaN &     NaN &    NaN &  permuted-DReG - DReG \\
                & mesquite & 16 &  2.67 &    0.53 &   0.74 &  permuted-DReG - DReG \\
                & radon & 16 &   NaN & 1167.95 & 269.26 &  permuted-DReG - DReG \\
                & wells & 16 &  0.04 &    0.02 &  -0.02 &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &        2 &        4 &        8 &                   measure \\
approxDist & model\_name & n &          &          &          &                           \\
\midrule
FullCovGaussian & election88 & 16 &      NaN &  2494.11 &  2197.37 &  complete-U - standard IW \\
                & election88Exp & 16 &      NaN &      NaN &      NaN &  complete-U - standard IW \\
                & irt & 16 & 19420.74 & 22057.71 & 17579.58 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &        2 &        4 &        8 &                    measure \\
approxDist & model\_name & n &          &          &          &                            \\
\midrule
FullCovGaussian & election88 & 16 &      NaN &  2494.14 &  2170.74 &  approx. 2nd - standard IW \\
                & election88Exp & 16 &      NaN &      NaN &      NaN &  approx. 2nd - standard IW \\
                & irt & 16 & 19399.79 & 22000.35 & 17686.39 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &        2 &        4 &        8 &                 measure \\
approxDist & model\_name & n &          &          &          &                         \\
\midrule
FullCovGaussian & election88 & 16 &      NaN &  1785.97 &  1133.70 &  permuted - standard IW \\
                & election88Exp & 16 &      NaN &      NaN &      NaN &  permuted - standard IW \\
                & irt & 16 & 17793.89 & 20064.36 & 16077.03 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &   2 &       4 &       8 &                 measure \\
approxDist & model\_name & n &     &         &         &                         \\
\midrule
FullCovGaussian & election88 & 16 & NaN & 2491.11 & 2123.90 &  complete-U-DReG - DReG \\
                & election88Exp & 16 & NaN &     NaN &     NaN &  complete-U-DReG - DReG \\
                & irt & 16 & NaN &     NaN &     NaN &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &   2 &       4 &       8 &               measure \\
approxDist & model\_name & n &     &         &         &                       \\
\midrule
FullCovGaussian & election88 & 16 & NaN & 1776.80 & 1116.11 &  permuted-DReG - DReG \\
                & election88Exp & 16 & NaN &     NaN &     NaN &  permuted-DReG - DReG \\
                & irt & 16 & NaN &     NaN &     NaN &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}


==> autogenerated/average-diff.tex <==
% this file was auto-generated
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                   measure \\
approxDist & model\_name & n &       &       &       &                           \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  0.01 &  0.36 &  0.55 &  complete-U - standard IW \\
                 & logistic-australian & 16 & -0.23 & -0.35 & -0.10 &  complete-U - standard IW \\
                 & logistic-ionosphere & 16 & -0.29 & -0.39 & -0.21 &  complete-U - standard IW \\
                 & logistic-madelon & 16 &  2.59 &  4.56 &  7.02 &  complete-U - standard IW \\
                 & logistic-mushrooms & 16 &  0.20 &  0.54 &  1.31 &  complete-U - standard IW \\
                 & logistic-sonar & 16 & -0.70 & -1.05 & -0.62 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                measure \\
approxDist & model\_name & n &       &       &       &                        \\
\midrule
DiagonalGaussian & logistic-a1a & 16 & -0.01 &  0.25 &  0.42 &  approx. - standard IW \\
                 & logistic-australian & 16 & -0.30 & -0.47 & -0.23 &  approx. - standard IW \\
                 & logistic-ionosphere & 16 & -0.34 & -0.50 & -0.34 &  approx. - standard IW \\
                 & logistic-madelon & 16 &  2.45 &  4.43 &  6.31 &  approx. - standard IW \\
                 & logistic-mushrooms & 16 &  0.15 &  0.47 &  1.18 &  approx. - standard IW \\
                 & logistic-sonar & 16 & -0.72 & -1.07 & -0.67 &  approx. - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                    measure \\
approxDist & model\_name & n &       &       &       &                            \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  0.01 &  0.31 &  0.50 &  approx. 2nd - standard IW \\
                 & logistic-australian & 16 & -0.26 & -0.40 & -0.14 &  approx. 2nd - standard IW \\
                 & logistic-ionosphere & 16 & -0.30 & -0.43 & -0.25 &  approx. 2nd - standard IW \\
                 & logistic-madelon & 16 &  2.51 &  4.39 &  6.94 &  approx. 2nd - standard IW \\
                 & logistic-mushrooms & 16 &  0.19 &  0.52 &  1.31 &  approx. 2nd - standard IW \\
                 & logistic-sonar & 16 & -0.70 & -1.04 & -0.65 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                       measure \\
approxDist & model\_name & n &       &       &       &                               \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  0.03 &  0.34 &  0.55 &  random subsets - standard IW \\
                 & logistic-australian & 16 & -0.22 & -0.34 & -0.08 &  random subsets - standard IW \\
                 & logistic-ionosphere & 16 & -0.25 & -0.36 & -0.18 &  random subsets - standard IW \\
                 & logistic-madelon & 16 &  2.42 &  4.25 &  6.21 &  random subsets - standard IW \\
                 & logistic-mushrooms & 16 &  0.14 &  0.58 &  1.05 &  random subsets - standard IW \\
                 & logistic-sonar & 16 & -0.64 & -0.95 & -0.56 &  random subsets - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                 measure \\
approxDist & model\_name & n &       &       &       &                         \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  0.04 &  0.34 &  0.54 &  permuted - standard IW \\
                 & logistic-australian & 16 & -0.23 & -0.34 & -0.07 &  permuted - standard IW \\
                 & logistic-ionosphere & 16 & -0.27 & -0.36 & -0.20 &  permuted - standard IW \\
                 & logistic-madelon & 16 &  2.60 &  4.18 &  6.52 &  permuted - standard IW \\
                 & logistic-mushrooms & 16 &  0.21 &  0.48 &  1.17 &  permuted - standard IW \\
                 & logistic-sonar & 16 & -0.66 & -0.99 & -0.59 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &                 measure \\
approxDist & model\_name & n &       &       &       &                         \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  0.03 &  1.21 &  1.39 &  complete-U-DReG - DReG \\
                 & logistic-australian & 16 & -0.25 & -0.49 & -0.12 &  complete-U-DReG - DReG \\
                 & logistic-ionosphere & 16 & -0.29 & -0.39 & -0.15 &  complete-U-DReG - DReG \\
                 & logistic-madelon & 16 &  1.37 &  1.85 &  2.76 &  complete-U-DReG - DReG \\
                 & logistic-mushrooms & 16 &  0.27 &  0.67 &  1.12 &  complete-U-DReG - DReG \\
                 & logistic-sonar & 16 & -0.71 & -1.07 & -0.71 &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &                & m &     2 &     4 &     8 &               measure \\
approxDist & model\_name & n &       &       &       &                       \\
\midrule
DiagonalGaussian & logistic-a1a & 16 &  0.02 &  1.21 &  1.37 &  permuted-DReG - DReG \\
                 & logistic-australian & 16 & -0.24 & -0.47 & -0.08 &  permuted-DReG - DReG \\
                 & logistic-ionosphere & 16 & -0.28 & -0.36 & -0.12 &  permuted-DReG - DReG \\
                 & logistic-madelon & 16 &  1.39 &  1.75 &  2.63 &  permuted-DReG - DReG \\
                 & logistic-mushrooms & 16 &  0.21 &  0.70 &  1.08 &  permuted-DReG - DReG \\
                 & logistic-sonar & 16 & -0.68 & -1.00 & -0.64 &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                   measure \\
approxDist & model\_name & n &         &         &         &                           \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   47.50 &  105.65 &  122.31 &  complete-U - standard IW \\
                & logistic-australian & 16 &    1.34 &    2.72 &    3.50 &  complete-U - standard IW \\
                & logistic-ionosphere & 16 &    0.42 &    1.37 &    2.24 &  complete-U - standard IW \\
                & logistic-madelon & 16 & 2362.74 & 4524.27 & 7812.86 &  complete-U - standard IW \\
                & logistic-mushrooms & 16 &   67.31 &  153.34 &  214.49 &  complete-U - standard IW \\
                & logistic-sonar & 16 &    4.67 &    8.90 &   14.00 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                measure \\
approxDist & model\_name & n &         &         &         &                        \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   47.38 &  105.01 &  121.85 &  approx. - standard IW \\
                & logistic-australian & 16 &    1.00 &    2.23 &    2.91 &  approx. - standard IW \\
                & logistic-ionosphere & 16 &    0.09 &    0.89 &    1.69 &  approx. - standard IW \\
                & logistic-madelon & 16 & 2370.34 & 4523.23 & 7831.39 &  approx. - standard IW \\
                & logistic-mushrooms & 16 &   67.20 &  153.14 &  213.63 &  approx. - standard IW \\
                & logistic-sonar & 16 &    4.36 &    8.41 &   13.25 &  approx. - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                    measure \\
approxDist & model\_name & n &         &         &         &                            \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   47.48 &  105.22 &  122.29 &  approx. 2nd - standard IW \\
                & logistic-australian & 16 &    1.06 &    2.37 &    3.22 &  approx. 2nd - standard IW \\
                & logistic-ionosphere & 16 &    0.17 &    1.03 &    1.95 &  approx. 2nd - standard IW \\
                & logistic-madelon & 16 & 2369.34 & 4521.43 & 7823.39 &  approx. 2nd - standard IW \\
                & logistic-mushrooms & 16 &   67.21 &  153.44 &  214.12 &  approx. 2nd - standard IW \\
                & logistic-sonar & 16 &    4.46 &    8.60 &   13.74 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                       measure \\
approxDist & model\_name & n &         &         &         &                               \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   42.90 &   98.64 &  108.40 &  random subsets - standard IW \\
                & logistic-australian & 16 &    1.27 &    2.55 &    3.28 &  random subsets - standard IW \\
                & logistic-ionosphere & 16 &    0.36 &    1.29 &    2.05 &  random subsets - standard IW \\
                & logistic-madelon & 16 & 2103.00 & 4295.63 & 7563.01 &  random subsets - standard IW \\
                & logistic-mushrooms & 16 &   61.37 &  143.50 &  199.34 &  random subsets - standard IW \\
                & logistic-sonar & 16 &    4.15 &    8.38 &   13.22 &  random subsets - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &       2 &       4 &       8 &                 measure \\
approxDist & model\_name & n &         &         &         &                         \\
\midrule
FullCovGaussian & logistic-a1a & 16 &   45.32 &  100.48 &  112.38 &  permuted - standard IW \\
                & logistic-australian & 16 &    1.31 &    2.60 &    3.36 &  permuted - standard IW \\
                & logistic-ionosphere & 16 &    0.39 &    1.32 &    2.14 &  permuted - standard IW \\
                & logistic-madelon & 16 & 2273.28 & 4398.00 & 7686.33 &  permuted - standard IW \\
                & logistic-mushrooms & 16 &   64.39 &  145.71 &  202.38 &  permuted - standard IW \\
                & logistic-sonar & 16 &    4.40 &    8.58 &   13.51 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &     2 &      4 &      8 &                 measure \\
approxDist & model\_name & n &       &        &        &                         \\
\midrule
FullCovGaussian & logistic-a1a & 16 & 25.56 & 218.08 &  95.18 &  complete-U-DReG - DReG \\
                & logistic-australian & 16 &  1.46 &   1.91 &   3.96 &  complete-U-DReG - DReG \\
                & logistic-ionosphere & 16 &  0.44 &   1.72 &   2.32 &  complete-U-DReG - DReG \\
                & logistic-madelon & 16 &   NaN &    NaN &    NaN &  complete-U-DReG - DReG \\
                & logistic-mushrooms & 16 & 94.50 & 191.15 & 173.92 &  complete-U-DReG - DReG \\
                & logistic-sonar & 16 &  4.63 &   8.92 &  19.19 &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &                & m &     2 &      4 &      8 &               measure \\
approxDist & model\_name & n &       &        &        &                       \\
\midrule
FullCovGaussian & logistic-a1a & 16 & 27.28 & 111.66 & 119.47 &  permuted-DReG - DReG \\
                & logistic-australian & 16 &  1.45 &   1.87 &   3.94 &  permuted-DReG - DReG \\
                & logistic-ionosphere & 16 &  0.42 &   1.57 &   2.06 &  permuted-DReG - DReG \\
                & logistic-madelon & 16 &   NaN &    NaN &    NaN &  permuted-DReG - DReG \\
                & logistic-mushrooms & 16 & 93.37 & 185.88 & 178.89 &  permuted-DReG - DReG \\
                & logistic-sonar & 16 &  4.28 &   8.80 &  18.99 &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                   measure \\
approxDist & model\_name & n &       &        &       &                           \\
\midrule
DiagonalGaussian & congress & 16 &  2.90 &   4.89 &  7.70 &  complete-U - standard IW \\
                 & election88 & 16 &  0.13 &   2.79 &  7.15 &  complete-U - standard IW \\
                 & election88Exp & 16 &  4.72 & 117.72 & 55.27 &  complete-U - standard IW \\
                 & electric & 16 &  0.22 &   1.62 &  4.63 &  complete-U - standard IW \\
                 & electric-one-pred & 16 &  0.46 &   0.23 & -2.45 &  complete-U - standard IW \\
                 & hepatitis & 16 &  2.10 & 156.68 &  1.89 &  complete-U - standard IW \\
                 & hiv-chr & 16 &  0.24 &   2.16 & 21.62 &  complete-U - standard IW \\
                 & irt & 16 &  0.13 &   0.44 &  0.60 &  complete-U - standard IW \\
                 & irt-multilevel & 16 & 29.74 &  54.46 & 52.88 &  complete-U - standard IW \\
                 & mesquite & 16 & -0.01 &   0.04 &  0.17 &  complete-U - standard IW \\
                 & radon & 16 &  1.94 &   2.72 & 25.63 &  complete-U - standard IW \\
                 & wells & 16 & -0.03 &  -0.04 & -0.06 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                measure \\
approxDist & model\_name & n &       &        &       &                        \\
\midrule
DiagonalGaussian & congress & 16 &  2.76 &   4.72 &  7.38 &  approx. - standard IW \\
                 & election88 & 16 &  0.14 &   2.78 &  7.11 &  approx. - standard IW \\
                 & election88Exp & 16 &  4.71 & 117.69 & 55.05 &  approx. - standard IW \\
                 & electric & 16 &  0.09 &   1.44 &  4.24 &  approx. - standard IW \\
                 & electric-one-pred & 16 &  0.35 &   0.09 & -2.63 &  approx. - standard IW \\
                 & hepatitis & 16 &  2.00 & 156.50 &  1.78 &  approx. - standard IW \\
                 & hiv-chr & 16 &  0.38 &   1.95 & 20.85 &  approx. - standard IW \\
                 & irt & 16 & -0.03 &   0.12 &  0.10 &  approx. - standard IW \\
                 & irt-multilevel & 16 & 31.25 &  45.43 & 59.86 &  approx. - standard IW \\
                 & mesquite & 16 & -0.32 &  -0.48 & -0.33 &  approx. - standard IW \\
                 & radon & 16 &  1.77 &   2.26 & 25.01 &  approx. - standard IW \\
                 & wells & 16 & -0.32 &  -0.54 & -0.58 &  approx. - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                    measure \\
approxDist & model\_name & n &       &        &       &                            \\
\midrule
DiagonalGaussian & congress & 16 &  2.89 &   4.76 &  7.63 &  approx. 2nd - standard IW \\
                 & election88 & 16 &  0.12 &   2.84 &  7.06 &  approx. 2nd - standard IW \\
                 & election88Exp & 16 &  4.72 & 117.75 & 55.25 &  approx. 2nd - standard IW \\
                 & electric & 16 &  0.16 &   1.54 &  4.52 &  approx. 2nd - standard IW \\
                 & electric-one-pred & 16 &  0.39 &   0.17 & -2.52 &  approx. 2nd - standard IW \\
                 & hepatitis & 16 &  2.05 & 156.58 &  1.86 &  approx. 2nd - standard IW \\
                 & hiv-chr & 16 &  0.34 &   2.11 & 21.72 &  approx. 2nd - standard IW \\
                 & irt & 16 &  0.02 &   0.23 &  0.28 &  approx. 2nd - standard IW \\
                 & irt-multilevel & 16 & 29.71 &  48.19 & 53.59 &  approx. 2nd - standard IW \\
                 & mesquite & 16 & -0.26 &  -0.34 & -0.11 &  approx. 2nd - standard IW \\
                 & radon & 16 &  1.93 &   2.49 & 25.75 &  approx. 2nd - standard IW \\
                 & wells & 16 & -0.25 &  -0.40 & -0.36 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                       measure \\
approxDist & model\_name & n &       &        &       &                               \\
\midrule
DiagonalGaussian & congress & 16 &  2.45 &   4.17 &  7.09 &  random subsets - standard IW \\
                 & election88 & 16 &  0.37 &   2.46 &  6.62 &  random subsets - standard IW \\
                 & election88Exp & 16 &  5.27 & 104.59 & 43.10 &  random subsets - standard IW \\
                 & electric & 16 &  0.27 &   1.51 &  4.17 &  random subsets - standard IW \\
                 & electric-one-pred & 16 &  0.21 &   0.00 & -2.00 &  random subsets - standard IW \\
                 & hepatitis & 16 & -0.31 &   1.69 &  1.60 &  random subsets - standard IW \\
                 & hiv-chr & 16 &  0.04 &   1.73 & 17.42 &  random subsets - standard IW \\
                 & irt & 16 &  0.13 &   0.45 &  0.49 &  random subsets - standard IW \\
                 & irt-multilevel & 16 & 35.70 &  27.60 & 46.45 &  random subsets - standard IW \\
                 & mesquite & 16 & -0.01 &   0.03 &  0.18 &  random subsets - standard IW \\
                 & radon & 16 &  1.96 &   4.69 & 13.10 &  random subsets - standard IW \\
                 & wells & 16 & -0.02 &  -0.03 & -0.06 &  random subsets - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &     4 &     8 &                 measure \\
approxDist & model\_name & n &       &       &       &                         \\
\midrule
DiagonalGaussian & congress & 16 &  2.50 &  4.60 &  7.32 &  permuted - standard IW \\
                 & election88 & 16 &  0.11 &  2.66 &  6.94 &  permuted - standard IW \\
                 & election88Exp & 16 &  0.80 & 98.47 & 32.76 &  permuted - standard IW \\
                 & electric & 16 &  0.26 &  1.53 &  4.31 &  permuted - standard IW \\
                 & electric-one-pred & 16 &  0.26 & -0.19 & -2.24 &  permuted - standard IW \\
                 & hepatitis & 16 &  0.90 & -0.07 &  0.65 &  permuted - standard IW \\
                 & hiv-chr & 16 &  0.16 &  2.03 & 15.83 &  permuted - standard IW \\
                 & irt & 16 &  0.11 &  0.42 &  0.50 &  permuted - standard IW \\
                 & irt-multilevel & 16 & 35.66 & 43.76 & 62.25 &  permuted - standard IW \\
                 & mesquite & 16 & -0.01 &  0.04 &  0.17 &  permuted - standard IW \\
                 & radon & 16 &  2.00 &  1.90 &  7.43 &  permuted - standard IW \\
                 & wells & 16 & -0.03 & -0.04 & -0.06 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &                 measure \\
approxDist & model\_name & n &       &        &       &                         \\
\midrule
DiagonalGaussian & congress & 16 &  2.74 &   4.91 &  7.46 &  complete-U-DReG - DReG \\
                 & election88 & 16 &  0.15 &   2.61 &  7.20 &  complete-U-DReG - DReG \\
                 & election88Exp & 16 & 28.60 & 116.22 & 54.83 &  complete-U-DReG - DReG \\
                 & electric & 16 &  0.18 &   1.65 &  4.84 &  complete-U-DReG - DReG \\
                 & electric-one-pred & 16 &  0.47 &   0.11 & -2.44 &  complete-U-DReG - DReG \\
                 & hepatitis & 16 &  0.63 &   1.84 &  1.94 &  complete-U-DReG - DReG \\
                 & hiv-chr & 16 &  0.18 &   1.19 & 20.19 &  complete-U-DReG - DReG \\
                 & irt & 16 &  0.07 &   0.33 &  1.17 &  complete-U-DReG - DReG \\
                 & irt-multilevel & 16 & 51.13 &  65.92 & 52.05 &  complete-U-DReG - DReG \\
                 & mesquite & 16 & -0.02 &   0.04 &  0.16 &  complete-U-DReG - DReG \\
                 & radon & 16 &  2.37 &   2.62 & 44.50 &  complete-U-DReG - DReG \\
                 & wells & 16 & -0.02 &  -0.05 & -0.10 &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                 &       & m &     2 &      4 &     8 &               measure \\
approxDist & model\_name & n &       &        &       &                       \\
\midrule
DiagonalGaussian & congress & 16 &  2.37 &   4.68 &  7.01 &  permuted-DReG - DReG \\
                 & election88 & 16 &  0.10 &   2.67 &  6.83 &  permuted-DReG - DReG \\
                 & election88Exp & 16 & -1.91 & 100.04 & 32.52 &  permuted-DReG - DReG \\
                 & electric & 16 &  0.24 &   1.56 &  4.62 &  permuted-DReG - DReG \\
                 & electric-one-pred & 16 &  0.29 &  -0.23 & -2.25 &  permuted-DReG - DReG \\
                 & hepatitis & 16 & -0.30 &   0.93 &  0.69 &  permuted-DReG - DReG \\
                 & hiv-chr & 16 & -0.08 &   1.45 & 12.90 &  permuted-DReG - DReG \\
                 & irt & 16 &  0.06 &   0.30 &  0.70 &  permuted-DReG - DReG \\
                 & irt-multilevel & 16 & 34.64 &  50.22 & 55.18 &  permuted-DReG - DReG \\
                 & mesquite & 16 & -0.06 &   0.03 &  0.17 &  permuted-DReG - DReG \\
                 & radon & 16 &  2.34 &   2.09 & 22.74 &  permuted-DReG - DReG \\
                 & wells & 16 & -0.02 &  -0.05 & -0.09 &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                   measure \\
approxDist & model\_name & n &       &         &        &                           \\
\midrule
FullCovGaussian & congress & 16 & 12.80 &   12.60 &  20.78 &  complete-U - standard IW \\
                & electric & 16 &   NaN &  -77.48 &  86.50 &  complete-U - standard IW \\
                & electric-one-pred & 16 & -0.97 &   -2.19 &  -2.03 &  complete-U - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  complete-U - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 320.88 &  complete-U - standard IW \\
                & mesquite & 16 &  0.53 &    0.26 &   0.26 &  complete-U - standard IW \\
                & radon & 16 &   NaN & 1316.92 & 304.19 &  complete-U - standard IW \\
                & wells & 16 &  0.00 &    0.00 &  -0.04 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                measure \\
approxDist & model\_name & n &       &         &        &                        \\
\midrule
FullCovGaussian & congress & 16 & 12.68 &   12.30 &  20.16 &  approx. - standard IW \\
                & electric & 16 &   NaN &  -85.02 &  90.41 &  approx. - standard IW \\
                & electric-one-pred & 16 & -1.01 &   -2.31 &  -2.22 &  approx. - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  approx. - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 322.35 &  approx. - standard IW \\
                & mesquite & 16 &  0.16 &   -0.29 &  -0.23 &  approx. - standard IW \\
                & radon & 16 &   NaN & 1312.94 & 306.54 &  approx. - standard IW \\
                & wells & 16 & -0.43 &   -0.55 &  -0.54 &  approx. - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                    measure \\
approxDist & model\_name & n &       &         &        &                            \\
\midrule
FullCovGaussian & congress & 16 & 12.32 &   12.56 &  20.45 &  approx. 2nd - standard IW \\
                & electric & 16 &   NaN &  -77.53 &  89.06 &  approx. 2nd - standard IW \\
                & electric-one-pred & 16 & -0.98 &   -2.24 &  -2.09 &  approx. 2nd - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  approx. 2nd - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 325.85 &  approx. 2nd - standard IW \\
                & mesquite & 16 &  0.20 &   -0.16 &  -0.03 &  approx. 2nd - standard IW \\
                & radon & 16 &   NaN & 1316.08 & 303.68 &  approx. 2nd - standard IW \\
                & wells & 16 & -0.35 &   -0.41 &  -0.32 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                       measure \\
approxDist & model\_name & n &       &         &        &                               \\
\midrule
FullCovGaussian & congress & 16 & 10.74 &   11.69 &  19.20 &  random subsets - standard IW \\
                & electric & 16 &   NaN & -181.37 &  86.61 &  random subsets - standard IW \\
                & electric-one-pred & 16 & -1.23 &   -2.93 &  -1.59 &  random subsets - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  random subsets - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 238.64 &  random subsets - standard IW \\
                & mesquite & 16 &  0.53 &    0.23 &   0.25 &  random subsets - standard IW \\
                & radon & 16 &   NaN & 1069.05 & 273.33 &  random subsets - standard IW \\
                & wells & 16 &  0.00 &    0.01 &  -0.04 &  random subsets - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                 measure \\
approxDist & model\_name & n &       &         &        &                         \\
\midrule
FullCovGaussian & congress & 16 & 11.61 &   12.01 &  19.78 &  permuted - standard IW \\
                & electric & 16 &   NaN &  -37.99 &  80.47 &  permuted - standard IW \\
                & electric-one-pred & 16 & -0.29 &   -2.28 &  -1.55 &  permuted - standard IW \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  permuted - standard IW \\
                & hiv-chr & 16 &   NaN &     NaN & 283.26 &  permuted - standard IW \\
                & mesquite & 16 &  0.51 &    0.23 &   0.25 &  permuted - standard IW \\
                & radon & 16 &   NaN & 1149.81 & 268.85 &  permuted - standard IW \\
                & wells & 16 &  0.00 &    0.01 &  -0.04 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &                 measure \\
approxDist & model\_name & n &       &         &        &                         \\
\midrule
FullCovGaussian & congress & 16 & 14.97 &   13.55 &  21.78 &  complete-U-DReG - DReG \\
                & electric & 16 &   NaN &  -75.07 &  47.72 &  complete-U-DReG - DReG \\
                & electric-one-pred & 16 & -0.95 &   -2.18 &  -2.04 &  complete-U-DReG - DReG \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  complete-U-DReG - DReG \\
                & hiv-chr & 16 &   NaN &     NaN &    NaN &  complete-U-DReG - DReG \\
                & mesquite & 16 &  0.54 &    0.15 &   0.14 &  complete-U-DReG - DReG \\
                & radon & 16 &   NaN & 1348.67 & 320.80 &  complete-U-DReG - DReG \\
                & wells & 16 &  0.01 &    0.00 &  -0.04 &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &       & m &     2 &       4 &      8 &               measure \\
approxDist & model\_name & n &       &         &        &                       \\
\midrule
FullCovGaussian & congress & 16 & 13.54 &   13.10 &  20.95 &  permuted-DReG - DReG \\
                & electric & 16 &   NaN &  -43.15 &  34.93 &  permuted-DReG - DReG \\
                & electric-one-pred & 16 & -0.27 &   -2.28 &  -1.55 &  permuted-DReG - DReG \\
                & hepatitis & 16 &   NaN &     NaN &    NaN &  permuted-DReG - DReG \\
                & hiv-chr & 16 &   NaN &     NaN &    NaN &  permuted-DReG - DReG \\
                & mesquite & 16 &  0.53 &    0.10 &   0.12 &  permuted-DReG - DReG \\
                & radon & 16 &   NaN & 1167.54 & 269.14 &  permuted-DReG - DReG \\
                & wells & 16 &  0.01 &    0.00 &  -0.04 &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &        2 &        4 &        8 &                   measure \\
approxDist & model\_name & n &          &          &          &                           \\
\midrule
FullCovGaussian & election88 & 16 &      NaN &  2493.62 &  2197.53 &  complete-U - standard IW \\
                & election88Exp & 16 &      NaN &      NaN &      NaN &  complete-U - standard IW \\
                & irt & 16 & 19403.24 & 22063.69 & 17578.36 &  complete-U - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &        2 &        4 &        8 &                    measure \\
approxDist & model\_name & n &          &          &          &                            \\
\midrule
FullCovGaussian & election88 & 16 &      NaN &  2493.64 &  2170.92 &  approx. 2nd - standard IW \\
                & election88Exp & 16 &      NaN &      NaN &      NaN &  approx. 2nd - standard IW \\
                & irt & 16 & 19384.82 & 22006.36 & 17688.48 &  approx. 2nd - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &        2 &        4 &        8 &                 measure \\
approxDist & model\_name & n &          &          &          &                         \\
\midrule
FullCovGaussian & election88 & 16 &      NaN &  1785.70 &  1133.92 &  permuted - standard IW \\
                & election88Exp & 16 &      NaN &      NaN &      NaN &  permuted - standard IW \\
                & irt & 16 & 17776.54 & 20072.33 & 16073.71 &  permuted - standard IW \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &   2 &       4 &       8 &                 measure \\
approxDist & model\_name & n &     &         &         &                         \\
\midrule
FullCovGaussian & election88 & 16 & NaN & 2490.62 & 2124.10 &  complete-U-DReG - DReG \\
                & election88Exp & 16 & NaN &     NaN &     NaN &  complete-U-DReG - DReG \\
                & irt & 16 & NaN &     NaN &     NaN &  complete-U-DReG - DReG \\
\bottomrule
\end{tabular}
\begin{tabular}{lllrrrl}
\toprule
                &     & m &   2 &       4 &       8 &               measure \\
approxDist & model\_name & n &     &         &         &                       \\
\midrule
FullCovGaussian & election88 & 16 & NaN & 1776.53 & 1116.34 &  permuted-DReG - DReG \\
                & election88Exp & 16 & NaN &     NaN &     NaN &  permuted-DReG - DReG \\
                & irt & 16 & NaN &     NaN &     NaN &  permuted-DReG - DReG \\
\bottomrule
\end{tabular}

